Effects of Interfaces on Human-Robot Trust: Specifying and Visualizing Physical Zones

In this paper we investigate the influence interfaces and feedback have on human-robot trust levels when operating in a shared physical space. The task we use is specifying a "no-go" region for a robot in an indoor environment. We evaluate three styles of interface (physical, AR, and map-based) and four feedback mechanisms (no feedback, robot drives around the space, an AR "fence", and the region marked on the map). Our evaluation looks at both usability and trust. Specifically, if the participant trusts that the robot "knows" where the no-go region is and their confidence in the robot's ability to avoid that region. We use both self-reported and indirect measures of trust and usability. Our key findings are: 1) interfaces and feedback do influence levels of trust; 2) the participants largely preferred a mixed interface-feedback pair, where the modality for the interface differed from the feedback.

==> Text/3.1surveyDesign.tex <==
\subsection{Survey design}
\label{sec:surveyDesign}



==> Text/3.2Participants.tex <==
\subsection{Participants}
\label{sec:participants}
Participants (30 total) consisted of Rhodes College faculty (16.7\%), staff (3.3\%), and students (80\%). 80\% of participants were 18-24 years old, with the remaining participants ranging from 36-60 years old. 30\% identified as women, and 70\% as men. As a group they tended to be tech-savvy, robot-friendly, and fairly comfortable with new technology.


==> Text/3.3DataAnalysis.tex <==
\subsection{Data Analysis}
\label{sec:analysis}




==> Text/3.oldmethod.tex <==
\section{Methods}
 The main goal of this research is to study how human trust is influenced when being exposed to different robotic interfaces and feedback conditions. We were specifically interested in learning how humans trust that a robot respects their privacy when they mark off a no-go region. Therefore, in our study we introduced 3 interfaces, 3 feedback conditions, 3 specification techniques and 3 tasks.
 
 \textbf{Interface} refers to the environment that we designed for the participants to interact with the robot. The proposed interfaces are: 1) Physical: Participants have a chance to be around the physical robot and see its actual performance. 2) AR: Participants will be presented with an Augmented Reality view of the world. 3) Map: Participants will be presented with a map that represents the actual study environment. 
 
\textbf{Specification} refers to the technique used to specify the no-go region when being introduced to the interfaces. In physical interface, the specification is placing four real, orange cones on the ground to mark the corners of the no-go region. In AR interface, specification refers to positioning of four virtual cones through an app by tapping the screen of a smartphone. In the map interface, specification refers to clicking four points on a map of the room to mark the corners of the no-go region. Figure \ref{fig:specification} illustrates the no-go region specification techniques.

\textbf{Feedback conditions} refer to the feedback that participants receive based on their interaction with the mentioned interfaces. The feedback that participants receive when interacting with the three interfaces varies due to their different nature. In physical interface, feedback is observing the robot driving around the room and avoiding the no-go region.
 In the AR interface, the feedback is the appearance of a virtual fence on the phone's screen where the no-go region was specified. In the map interface the feedback is specifying the no-go region on a map of the room by red shading. Figure \ref{fig:feedback} presents all the feedback conditions.

\textbf{Tasks} Overall, the experiment consists of three tasks. Task 1 aims to learn about participants' trust by directly asking them to specify a safe region inside the no-go region that they believe the robot will no enter. 
Task 2 aims to learn about participants' trust by indirectly asking them to place items with different levels of fragility to rank the safety of three predefined areas inside the no-go region. Task 3 investigates what interface participants prefer the most and possible reasons of their interface preferences. 
\input{Text/SpecificationPictures.tex}
\input{Text/FeedbackPictures.tex}
 %In this study, we examine the effect that three different interfaces (i.e. Physical, Map, and AR) and four feedback conditions (i.e. Physical, Map, AR, and none) for creating private regions have on people’s trust in a robot and their interface preference. 

%The experiment consisted of three tasks. A random interface was assigned to participants for the first and second tasks, and a random feedback condition was also assigned to participants for the first task. In the third task, all three interfaces were shown to participants, and the three feedback conditions were explained to them. Participants were allowed to choose one interface to use and one feedback condition to be shown to them.


 
%  \subsection{Conditions}
%  We created three interfaces for specifying a private, no-go region for the robot:
%  \begin{enumerate}
%     \item Physical: Four real, orange cones are placed on the ground to mark the corners of the no-go region.
%     \item Map: Four points are clicked on a map of the room to mark the corners of the no-go region.
%     \item AR: Four virtual cones are positioned through an app by tapping the screen of a smartphone.
% \end{enumerate}

% After a no-go region is created, four different feedback conditions are available to demonstrate the effectiveness of the no-go region to the user:
% \begin{enumerate}
%     \item Physical: The robot drives around the room and avoids the no-go region.
%     \item Map: The no-go region is shaded red on a map of the room.
%     \item AR: A virtual fence appears on the phone's screen where the no-go region was specified.
%     \item Control:  No feedback is provided.
% \end{enumerate}


\subsection{Procedure}

Participants started the study by providing answers to an entry survey\footnote{Entry survey: \url{https://forms.gle/b5vfFUPmAGWah5gX8}} consisting of standard demographic questions and questions that evaluated their initial attitude toward robots, the latter of which were drawn from the Negative Attitudes towards Robots Survey \cite{Nomura2004Nars}. Then, they proceed to the three tasks. 

\textbf{Task 1:} In task 1 the study coordinator showed the participant how to create a no-go region with our proposed interfaces and set the no-go region herself. She explained that the robot will not enter the region. 
\begin{itemize}
    \item Physical Interface: Study coordinator first presents the physical interface by introducing the robot and specifying the no-go region by placing four real orange cones. In this scenario participants once observed the robot driving around the room and avoiding the no-go region. Then participants were told to specify a safe place inside a the no go region so that a rickety table that had a fragile item on top of it was safe from robot's possible collision. The study coordinator asked the participants to move the table throughout all the areas of the no-go region that they would feel comfortable leaving the table.
    \item AR Interface: After presenting the physical interface, the study coordinator introduces the AR interfaces and specifies the no-go region by placing four virtual cones. Upon appearance of the virtual cones, AR places virtual fences to connect the virtual cones. Participants were told that robot respects can recognize the virtual wall and it will avoid going through them. Again we ask the participants to specify  a safe place inside a the no go region so that a rickety table that had a fragile item on top of it was safe from robot's possible collision. The study coordinator asked the participants to move the table throughout all the areas of the no-go region that they would feel comfortable leaving the table.
    \item Map: After presenting the AR interface, the study coordinator introduces the map interfaces and specifies the no-go region by clicking four points on a map of the study environment. Upon appearance of the four points on the map, map interface shades red the no-go region. Participants were told that robot respects a no-go region specified on the map and it will avoid going into it. We asked the participants to specify a safe place inside a the no-go region using the map (participants can click on the map and put dots to illustrate the safe region) so that a rickety table that had a fragile item on top of it was safe from robot's possible collision. The study coordinator asked the participants to tap on the map to specify all the areas of the no-go region that they would feel comfortable leaving the table.
\end{itemize}



% Then, the participant was shown one of the three feedback conditions. The experimenter presented the participant with a rickety table that had a fragile item on top of it and told the participant that if the robot bumped into the table, the fragile item might fall and break. The study coordinator asked the participant to move the table throughout all the areas of the no-go region that they would feel comfortable leaving the table.


% Participants were asked to complete three surveys and three tasks. First, they were given an entry survey\footnote{Entry survey: \url{https://forms.gle/b5vfFUPmAGWah5gX8}} consisting of standard demographic questions and questions that evaluated their initial attitude toward robots, the latter of which were drawn from the Negative Attitudes towards Robots Survey \cite{Nomura2004Nars}.

% Once the participants finished the survey, the study coordinator showed the participant how to create a no-go region with one of the interfaces and explained that the robot should not enter the region. Then, the participant was shown one of the three feedback conditions. The experimenter presented the participant with a rickety table that had a fragile item on top of it and told the participant that if the robot bumped into the table, the fragile item might fall and break. The study coordinator asked the participant to move the table throughout all the areas of the no-go region that they would feel comfortable leaving the table. 

\textbf{Task 2:} In the second task, the no go region is the same as what it was in Task 1. The study coordinator placed three tables inside a no-go region that had been created using one of the interfaces. The study coordinator then presented the participant with six items (two durable, two normal, and two fragile) (Figure \ref{fig:items}) and asked the participant to place the items on the tables so that they are visible to people in the room and also safe from being knocked off by the robot.

\begin{itemize}
    \item Physical interface: Participants were asked to physically place the items on the three tables.
    \item AR interface: Participants could either physically place the items on the table or just tell how they would place the items.
    \item Map interface: Three tables were shown in the map, and participants showed which table is the best place to put each item by tapping on the tables in the map.
\end{itemize}
% For the second task, the study coordinator placed multiple tables inside a no-go region that had been created using one of the specified methods. The study coordinator then presented the participant with three items (one durable, one normal, and one fragile) and asked the participant to place the items on the tables so that they are visible to people in the room and also safe from being knocked off by the robot.
\input{Text/task2Items}
% picture frames? display items? put liquid in the cups?

After the second task, participants were given the mid-study survey\footnote{Mid-Study survey: \url{https://forms.gle/WoZ3i9BdzzVCewN36}} which evaluated their confidence that the robot would avoid the no-go region when being exposed to the three interfaces. 

\textbf{Task 3:} In the third task, participants were asked to select their most desirable interface among all the three interfaces (i.e. the interface that is most capable of stopping the robot from going through the no-go region) and create a no-go region using their respective no-go region specification technique. Then, study coordinator presents the participants with the six items (two durable, two normal, and two fragile) and ask them to place the items in any place that they feel safe that the robot would not bumped into. Participants were free place these items anywhere (e.g. inside the no-go region, outside the no-go region). Moreover, they could move the objects in the study area (e.g. cones, chairs, tables, shelves,...) to make them more comfortable that the items are safe in the environment. 

% Next, the study coordinator placed a rickety table with a fragile item on top of it in the room and asked the participant to create a no-go region using a method of their choosing. Upon the selection of their desirable interface and specification technique, their chosen interface presents the feedback technique.


% In the third task, participants were introduced to all three methods for creating a no-go region and the three feedback methods. Next, the study coordinator placed a rickety table with a fragile item on top of it in the room and asked the participant to create a no-go region using a method of their choosing. The study coordinator then showed the participant the feedback method that they chose. 

Finally, the participant was given an exit survey,\footnote{Exit survey: \url{https://forms.gle/FQEL8t1xzPoj4SYf8}} the first part of which repeated questions from the mid-study survey. The remaining part of the exit survey assessed the participant’s trust in the robot’s abilities. 

\subsection{Measures}
We measure the participants' trust in the robot both directly and indirectly. In Task 1, the distance from the table to the edge of the no-go region is recorded, with a shorter distance meaning higher trust that the robot will recognize and avoid the no-go region. Similarly, in task 2, the location of the tables that items are placed on as well as the placement of the items themselves are both noted. High trust that the robot will avoid the no-go region is indicated when an item is placed on a table that is close to the edge of the no-go region and when an item is placed close to the edge of the table itself. 

The three surveys directly measure participants' trust. The entry survey contains questions from NARS to determine participants' initial attitude toward robots. Both the mid-study and exit surveys ask participants to rate the robot's ability to do specified tasks. In addition, the exit survey directly asks participants how much they trust the robot to perform certain tasks and what would make them more or less likely to trust the robot.

We also measure user preference in the third task by recording which interface and feedback condition participants choose.




==> Text/6.limitations.tex <==
\section{Limitations}



==> Text/8.acknowledgment.tex <==
\section{Acknowledgment}

Funded in part by NSF grants NRI 2024872 and 2024673.

==> Text/FeedbackPictures.tex <==
\begin{figure}[ht]
\centering
\minipage{0.45\textwidth}
  \includegraphics[width=\linewidth]{Figures/Physical_Feedback_Annotated.png}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.325\textwidth}
  \includegraphics[width=\linewidth]{Figures/MapFeedback1.png}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.225\textwidth}
  \includegraphics[width=\linewidth]{Figures/AR_Feedback1.PNG}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Feedback Conditions: \textbf{(a)} Physical
\textbf{(b)} Map
\textbf{(c)} AR}
\label{fig:feedback}
\end{figure}

==> Text/Old styles/ConferenceLink.tex <==
http://www.colips.org/conferences/icsr2021/wp/call-for-papers/


==> Text/ResultsFigures/H1H2T2.tex <==
\begin{figure*} [!h]
    \centering
    \minipage{0.5\linewidth}
        \includegraphics[width=\linewidth]{Figures/Results/obj_placement.pdf}
    \endminipage
    \minipage{0.40\linewidth}
        \includegraphics[width=\linewidth]{Figures/Results/Trust_obj1.pdf}
    \endminipage
\caption{Object placement on close vs far table per interface \textbf{(left)} Object distances per feedback \textbf{(right).}}
\label{fig:Task2Measures}
\end{figure*}

==> Text/ResultsFigures/H1T2.tex <==
\begin{figure} [h]
\centering
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T2Obj1PlacementInterface.pdf}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T2Obj1PlacementInterface.pdf}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T2Obj1PlacementInterface.pdf}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Task 2 Object Placement: \textbf{(a)} Fragile
\textbf{(b)} Normal
\textbf{(c)} Durable}
\label{fig:T2ObjPlacementInterface}
\end{figure}

%\begin{wrapfigure}{R}{0.5\textwidth}
%    \centering
%    \vspace{-20pt}
%    \includegraphics[width=0.48\textwidth]{Figures/Results/T2ObjDistancesInterface.pdf}
%    \caption{Task 2: Average Distance to Edge of Table by Object}
%    \label{fig:T2InterfaceDistance}
%\end{wrapfigure}
\begin{figure} [h]
\centering
\minipage{0.5\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/T2ObjDistancesInterface.pdf}
\endminipage
\caption{Task 2: Average Distances of Objects to Edge of Table}
\label{fig:T2InterfaceDistance}
\end{figure}

==> Text/ResultsFigures/H1T3-1.tex <==
\begin{figure} [h]
\centering
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1InterfaceDistance.pdf}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1InterfaceArea.pdf}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1InterfaceArea.pdf}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Task 3-1 Measures: \textbf{(a)} Avg Distance of Table to Edge of No-Go Region
\textbf{(b)} Avg Area of No-Go Region
\textbf{(c)} Avg Ratio of Area of No-Go Region to Area of Table}
\label{fig:T3-1FiguresInterface}
\end{figure}

==> Text/ResultsFigures/H1T3-2.tex <==
\begin{figure} [h]
\centering
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2InterfaceDistance.pdf}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2InterfaceArea.pdf}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2InterfaceArea.pdf}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Task 3-2 Measures: \textbf{(a)} Avg Distance of Table to Edge of No-Go Region
\textbf{(b)} Avg Area of No-Go Region
\textbf{(c)} Avg Ratio of Area of No-Go Region to Area of Table}
\label{fig:T3-2FiguresInterface}
\end{figure}

==> Text/ResultsFigures/H2T1.tex <==
%\begin{wrapfigure}{r}{0.5\textwidth}
%    \centering
%    \vspace{-30pt}
%    \includegraphics[width=\linewidth]{Figures/Results/T1FeedbackDistance.pdf}
%    \caption{Task 1: Average Distance from Table to Edge of No-Go Region}
%    \label{fig:T1FeedbackDistance}
%\end{wrapfigure}
\begin{figure} [h]
\centering
\minipage{0.5\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/T1_tabledist_fb.png}
\endminipage
\minipage{0.5\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/T1_tabledist_combo.png}
\endminipage
\caption{Task 1: Average Distance from Table to Edge of No-Go Region}
\label{fig:T1FeedbackDistance}
\end{figure}

==> Text/ResultsFigures/H2T2.tex <==
\begin{figure} [h]
\centering
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T2Obj1PlacementFeedback.pdf}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T2Obj1PlacementFeedback.pdf}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T2Obj1PlacementFeedback.pdf}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Task 2 Object Placement: \textbf{(a)} Fragile
\textbf{(b)} Normal
\textbf{(c)} Durable}
\label{fig:T2ObjPlacementFeedback}
\end{figure}

%\begin{wrapfigure}{r}{0.5\textwidth}
%    \centering
%    \vspace{-20pt}
%    \includegraphics[width=0.48\textwidth]{Figures/Results/T2ObjDistancesFeedback.pdf}
%    \caption{Task 2: Average Distance to Edge of Table by Object}
%    \label{fig:T2FeedbackDistance}
%\end{wrapfigure}
\begin{figure} [h]
\centering
\minipage{0.5\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/T2ObjDistancesFeedback.pdf}
\endminipage
\minipage{0.5\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/T2ObjDistancesCombo.pdf}
\endminipage
\caption{Task 2: Average Distance to Edge of Table by Object}
\label{fig:T2FeedbackDistance}
\end{figure}

==> Text/ResultsFigures/H2T3-1.tex <==
\begin{figure} [h]
\centering
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1FeedbackDistance.pdf}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1FeedbackArea.pdf}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1FeedbackArea.pdf}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Task 3-1 Measures by Feedback: \textbf{(a)} Avg Distance of Table to Edge of No-Go Region
\textbf{(b)} Avg Area of No-Go Region
\textbf{(c)} Avg Ratio of Area of No-Go Region to Area of Table}
\label{fig:T3-1FiguresFeedback}
\end{figure}

\begin{figure} [h]
\centering
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1ComboDistance.pdf}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1ComboArea.pdf}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-1ComboArea.pdf}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Task 3-1 Measures by Interface/Feedback Combo: \textbf{(a)} Avg Distance of Table to Edge of No-Go Region
\textbf{(b)} Avg Area of No-Go Region
\textbf{(c)} Avg Ratio of Area of No-Go Region to Area of Table}
\label{fig:T3-1FiguresCombo}
\end{figure}

==> Text/ResultsFigures/H2T3-2.tex <==
\begin{figure}[h]
\centering
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2FeedbackDistance.pdf}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2FeedbackArea.pdf}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2FeedbackArea.pdf}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Task 3-2 Measures by Feedback: \textbf{(a)} Avg Distance of Table to Edge of No-Go Region
\textbf{(b)} Avg Area of No-Go Region
\textbf{(c)} Avg Ratio of Area of No-Go Region to Area of Table}
\label{fig:T3-2FiguresFeedback}
\end{figure}

\begin{figure}[h]
\centering
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2ComboDistance.pdf}
  \centering
  \textbf{(a)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2ComboArea.pdf}
  \centering
  \textbf{(b)}
\endminipage
\minipage{0.30\textwidth}
  \includegraphics[width=\linewidth]{Figures/Results/T3-2ComboArea.pdf}
  \centering
  \textbf{(c)}
\endminipage
\caption{ Task 3-2 Measures by Interface/Feedback Combo: \textbf{(a)} Avg Distance of Table to Edge of No-Go Region
\textbf{(b)} Avg Area of No-Go Region
\textbf{(c)} Avg Ratio of Area of No-Go Region to Area of Table}
\label{fig:T3-2FiguresCombo}
\end{figure}

==> Text/ResultsFigures/H4.tex <==
\begin{figure}[h]
\centering
\minipage{0.50\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/FeedbackPreference.png}
    \centering
    \textbf{(a)}
\endminipage
\minipage{0.50\textwidth}
    \includegraphics[width=\linewidth]{Figures/Results/ComboPreference.png}
    \centering
    \textbf{(b)}
\endminipage
\caption{ \textbf{(a)} Feedback Preference in Task 3-2
\textbf{(b)} Interface/Feedback Combination Preference}
\label{fig:FeedbackPreference}
\end{figure}

==> Text/TODOs.tex <==
[Done] Figures 1, 2 & 3: 
   -[Done] Ditch the sub labels and put the labels on the images themselves
   -[Done] combine 1 & 2
   -[Done] figure 3 should be labeled as 1,2,3,4  & fragile vs durable
        - stack fragile images, durable images, side by side with table
        - Caption is objects & tables for task 2. (one table used task 1)
   -[Done] add picture of tables to figure 3 - label close, far, draw cones in, draw distance measure
   - [Done]in section 3.2 add reference to figures
   - [Done]It bothers me a little bit that we cannot see the 4th cone in the AR interface image.  Retake? We'll try

[Done] Fix survey measure text
   - describe likert scale How?  What needs to be done?

[Done] For task 1/2 was there a request to make things visible? Place where safe

[Done] Sanity check region size with interface
We can do that.  What do we want to add to the paper?
- add a sentence to methods that says: To make sure the interfaces were comparable, we pilot studied with ease of use, time to specify region. We also verified that they came out roughly the same size (+- 4%)

[Done] -put in the feedback section how long it takes for the robot to drive around the region

[Done] For task 3, was there a place the table in the middle (did they place or just draw around, could they move it after?) and were they told to make as small as possible?

[Done] 
  - [Done] combine figures into pdf and post somewhere and include a link: here https://docs.google.com/document/d/15hgv0uLz1QcIYzeA1khDp15WrSXCog8qNoWvNaMS84I/edit#heading=h.35hkvq11okto
  - [Done] Missing NARS and attitude towards robot plots
Figure out if we want to add a figure of the results for h1/h2. Could do the summary of the survey results with the summary of the object distances and close/far, by all 6 conditions. It might fit.


[Marisa - if easy to do t-tests, then annotate figures in supplemental ]Maybe a t-test for table and area of region
Make sure we know what data we are performing t-test on and where we want to report p-value in paper
[If we can do t-tests for table distance task 1, task 3.1 and 3.2, table area for 3.1 and 3.2] - add a footnote or note to section 4.1 about which of these averages are statistically significant.
[Survey data for changing their mind - shift from feedback to no feedback, the 3 interfaces] Section 4.1

[Bill] Add a sentence or two to summarize key findings to the abstract, conclusion

[Sogol ]Do we really have 54 cites?  Or is nocite turned on or something?  We need to get this down to one page instead of 3+.  Also ditch all of the doi https information, trim cites down

[Sogol] There is no transition from related work to methods.  I feel like we need a couple of sentences that situate our contribution in this paper in relation to the existing literature. Add bridging structure to our study - what is our contribution to the related work. 

[Done] Add more to the discussion -- Limitations?  Threats to generalizability?
 - limitations:
    - Our study took place in a staged environment.  It had the look and feel of an office lounge area, but the user did not own the furniture, objects, or the robot.  We cannot be certain that our results would extend to a person's real living room or office.
    - We tested three different types of interfaces, but there may be additional interfaces that could be developed that would potentially be more effective for particular tasks.  
    - Novelty effect -- use it because it's new, use it once -- physical driving around is great once, but it takes time.  
    - Only measuring trust in the first encounter.  Not considering longitudinal, over time, how trust gets built.  
    - Add a sentence in discussion about the fact that you can't see the table in the map interface (harder to put tight boundary because you don't know where the table is)

[Bill] Write conclusions

[Cindy] For Acknowledgment, do we reference the NSF grant?  It certainly supported this work, even if it is only tangentially related to the actual grant. Yes
[Bill] Do you want to add the Ebola since it funded sogol in part?

[Done] There does not seem to be a supplemental materials submission for this conference.  We already have a url footnote for the entry survey.  I suppose we could footnote any other supplemental stuff we wanted the reviewers to be able to access.  
--Put it here?  
http://cs.rhodes.edu/~sowellr/research/trust/survey.pdf

[Bill] Get Bill to read.  Fresh eyes will be helpful to make sure we're telling a coherent story.  

[Done] Squish. Help us get it down to 10 pages.

[Done] Tweak Figures 1 and 2.  Adjust the labels -- make the text boxes tighter and slightly transparent. 

[Ross] Submit

==> Text/reviews.tex <==
Gmail	Ross Sowell <rsowell@gmail.com>
[EXTERNAL] [ICSR2021] Paper decision status for paper 006
1 message
ICSR2021 (via OCS) <noreply@springer.com>	Mon, Aug 30, 2021 at 7:42 AM
Reply-To: "hongsheng.he@wichita.edu" <hongsheng.he@wichita.edu>
To: Sowell_Ross <sowellr@rhodes.edu>
Dear Ross Sowell,

We regret to inform you that your paper

        006 -- 'Engendering Human-Robot Trust: Specifying and Visualizing Physical Privacy Zones'

was rejected to appear in the conference

        'The 13th International Conference on Social Robotics (ICSR 2021)'.

Enclosed please find the reports.

Final Report:

ARGUMENTATION:

We regret to inform you that your paper has not been accepted for publication at the 13th International Conference on Social Robotics (ICSR 2021). The conference received many quality papers and unfortunately not all of them could be accepted.

A total of 129 papers were submitted for review this year. 64 were selected for full paper publication (49.6% acceptance rate), while 18 more papers were selected as Brief Research Reports. Each submission was reviewed by at least two Program Committee members and provided with a summary report from a Senior Program Committee member. Based on these reviews and reports, the Program Chairs made the final decisions.

The conference will be held on November 10-13, 2021 as a hybrid conference. More information on the conference can be found at the conference website (www.colips.org/conferences/icsr2021).

Thank you again for submitting your paper to ICSR! Although this paper was not accepted, we are still looking forward to meeting you at ICSR 2021 in person or online.

Yours sincerely,

Yan Wu, Agnieszka Wykowska, and Hongsheng He
Program Chairs

Haizhou Li and Shuzhi Sam Ge
General Chairs



Reports:

---------------

ARGUMENTATION:

Meta review.
The authors found the subject of this paper interesting, novel and timely. They praised the efforts of the authors for the in-person study with a real robot.
However, both reviewers raised weaknesses and limitations in the paper, form the structure of the paper (unconventional introduction), the study design, and the report of the results. R2 also raised that the term “privacy” in the title did not reflect in the manuscript.
In addition, R2 does not believe that the robot in the present study is “social”, which makes it not adequate for the conference.
Both reviewers took the decision to weakly reject the manuscript for the conference.


###
R1.
+ Summary +
Participants (N=30) in a 3(interface: AR, map or non-virtual cones) x2 (feedback/none) repeated measures study performed 4 separate tasks: placing a fragile table+object in a no-go region, placing fragile and non-fragile objects on near and far pre-placed tables in a no-go region, creating a no-go region and picking an interface. Results showed participants placed fragile objects further from the robot, preferred the AR interface over all other interfaces and trusted the cones and AR-marked no-go regions more than the map.

The only issue with this paper is they are missing statistical tests. It’s an interesting paper.

+ Strengths +
Did an in-person study with real robot and participants
Collected both survey and behavioral data, and novel measures were collected, including table distance and object position
Novel experiment design of no-go region and balancing of conditions and gathered data on 4 different tasks

+ Weaknesses +
Organization issues – the Intro doesn’t sufficiently introduce the topic but rather offers a description of methodology and lists hypotheses
Insufficient explanation of the hypotheses and past work/value of addressing no-go regions
No statistical tests presented in Results

+ Suggestions +
Use statistical quantitative analysis to replace more qualitative statements of comparative differences
Improve the strength of the results by including only statements with statistical validity, e.g, Fig. 3 looks like there’s no significant difference between map and physical, but the comparison of means in the main text suggests there is
Add to Discussion whether the feedback conditions that don’t involve a robot (i.e. Map/AR) can really represent a person’s trust in a robot

+ Minor points +
3rd row of Figure 3 doesn’t match main text
Could add more explanation about why the robot’s no-go interface would affect trust in the robot’s ability to navigate versus an ability for a user to specify coordinates in 2d space


###
R2.

This paper conducted a user study to investigate how interfaces (physical, GUI, and augmented reality) and feedback (physical, GUI, AR, and no feedback) could influence people's trust in and preference for the robot. Although I believe that people's trust to robot's ability of not invading "no-go" zone is important and the research questions posed by the authors are quite interesting, I have reservations on recommending the acceptance of this paper for the following reasons:

1) I did some research on the definitions of social robotics, and as far as I am concerned, the robot in this paper is not social. Social robots usually fall under the category of ‘proximate interaction’, in which ‘humans and robots interact as peers or companions.’ They were perceived as beings with thoughts, feelings, social awareness of the environment, capability to respond to users in a social manner, and capability to cause people's emotional responses. In other words, not every robot that people trust or distrust is social: people even trust/distrust machines that not are programmable based on the machines' competency. Thus, I believe this paper may not be a good fit for ICSR.
2) The experiment design of this paper seems to be confusing at least for me. Although the author included four different feedback options in the experiments, the experiment design only took two options into consideration: with feedback and without feedback. Since feedback modes can be one important factor influencing participants' trust and preference for the robot, it is important to block all the four conditions when studying "interface" categories, and vice versa. There are also several other problems with experiment design such as the "virtual fence" employed in AR condition but not in GUI condition. This is a confounding variable.
My best guess is that the author paired physical interface with physical feedback, GUI (map interface) with map feedback, and AR interface with AR feedback. However, the authors also paired all three interface conditions with no feedback. This is where the confusion comes into the picture for experiment design: 6 different pairs for a Latin Square Experiment Design of two variables. As I mentioned, the "feedback" variable has 4 levels instead of 2 levels in this experiment.
Another problem with the experiment design is how authors use "mixed method" design in this user study. As far as I understand, "mixed method" is used in the way that when one independent variable is experimented with between-group design, the other independent variable is experimented with within-group design. It is not about one independent variable experimented with a mix of within and between subject experiment design. Correct me if I am wrong, but I have never seen this kind of experiment design before, and I really do not know how to apply statistics analysis to a variable whose data is gathered through both within and between subject designs.
3) For the data analysis and results, my best guess is that there are 14 participants. However, theoretically, there are in general 3*4 = 12 experiment conditions (3 kinds of interfaces and 4 kinds of feedback) when treating "interface" and "feedback" as two variables. Even if there are 6 conditions and each condition is tested by 5 participants, I still do not see potential for enough statistical generalization powers to the results. Moreover, there is no statistics analysis to indicate whether the results are generalizable.
In addition, the authors use percentage comparison a lot during analysis and did not probe into the reasons behind "preference" and "trust" differences for different conditions. This means the authors are not focusing on qualitative feedback/results. For quantitative results, however, showing percentage only is not enough as proper statistics analysis. My suggestion would be focusing on the qualitative reasons and feedback for each paired conditions for this paper.
4) Finally, the structure of this paper is kind of unconventional. For introduction section, I don't get the context of this research, I don't understand why there are "no-go" zones or what tasks this mobile robot is performing for what user groups in what scenarios. I suggest authors to follow a more conventional introduction structure which gives contexts and background of this research. I also don't understand why authors borrowed three experiment conditions from Rueben et al. since that article focuses on Privacy, while this paper focuses on Trust and preference. Btw, I know the title of this paper has "physical privacy" in it, but I don't really see the content of this paper is closely related to privacy. I suggest authors citing more works related to "robot trust and preference" to backup the choice of different levels of interventions.
For the related work part, although I really appreciate the general review on robot trust and its measuring scales, I would like to see something more specific to the research topic of this paper. For instance, works about "no-go" zone, works that use interaction modalities or interaction modes as experiment conditions for robot trust and preference, works that investigate comparisons among GUI, physical interface, and AR interface, etc.
Btw, if you are doing a review on scales measuring robot trust, as far as I know, you probably need to mention "Bertram F. Malle" who did very solid works in this area. He joined the ROMAN-SCRITA workshop last year and I believe he is an expert in this.


---------------




--
This message was generated automatically by
- The Online Conference System (OCS) -

https://ocs.springer.com/ocs/



This email was sent from a non-Rhodes email address.
Please do not click links or open attachments unless you recognize the sender and are positive the content is safe.



